Convolutional Neural Bandit for Visual-aware Recommendation

Online recommendation/advertising is ubiquitous in web business. Image displaying is considered as one of the most commonly used formats to interact with customers. Contextual multi-armed bandit has shown success in the application of advertising to solve the exploration-exploitation dilemma existing in the recommendation procedure. Inspired by the visual-aware recommendation, in this paper, we propose a contextual bandit algorithm, where the convolutional neural network (CNN) is utilized to learn the reward function along with an upper confidence bound (UCB) for exploration. We also prove a near-optimal regret bound $\tilde{\mathcal{O}}(\sqrt{T})$ when the network is over-parameterized, and establish strong connections with convolutional neural tangent kernel (CNTK). Finally, we evaluate the empirical performance of the proposed algorithm and show that it outperforms other state-of-the-art UCB-based bandit algorithms on real-world image data sets.

==> analysis2copy.tex <==



\section{Proof of Lemma 6.2}

\begin{definition} \label{def:ridge}
Given the context vectors $\{\bx_i\}_{i=1}^t$ and the rewards $\{ r_i \}_{i=1}^{t} $, then we define the estimation $\widehat{\btheta}_0$ via ridge regression:  
\[
\begin{aligned}
&\mathbf{A}_0 =  \lambda \mathbf{I} + \sum_{i=1}^{t} g(\bx_i; \btheta^{(0)}) g(\bx_i; \btheta^{(0)})^\intercal /m \\
&\mathbf{b}_0 = \sum_{i=1}^t r_t g(\bx_i; \btheta^{(0)})  /\sqrt{m}\\
&\widehat{\btheta}_0 = \mathbf{A}^{-1}_0\mathbf{b}_0 
\end{aligned}
\]
\end{definition}
\iffalse
\begin{definition} \label{def:ridge}
Given the context vectors $\{\bx_i\}_{i=1}^t$ and the rewards $\{ r_i \}_{i=1}^{t} $, then we define the estimation $\bar{\btheta}_0$ via linear regression:  
\[
\begin{aligned}
&\mathbf{A}_0 =  \sum_{i=1}^{t} \gx{0}{i} \gx{0}{i}^\intercal /\sqrt{m}\\
&\mathbf{b}_0 = \sum_{i=1}^t r_t \gx{0}{i} /\sqrt{m}\\
&\bar{\btheta}_0 = \mathbf{A}^{-1}_0\mathbf{b}_0 
\end{aligned}
\]
\end{definition}
\fi











\begin{definition}
\[
\begin{aligned}
&\mathbf{G}^{(k)} = \left( g(\bx_1; \btheta^{(k)}), \dots,   g(\bx_t; \btheta^{(k)})\right)\\
&\mathbf{G}^{(0)} = \left( g(\bx_1; \btheta^{(0)}), \dots,   g(\bx_t; \btheta^{(0)})\right)\\
&\mathbf{f}^{(k)} = \left( f(\bx_1; \btheta^{(k)}), \dots,   f(\bx_t; \btheta^{(k)})    \right)^\intercal \\
& \mathbf{r} = \left( r_1, \dots, r_t  \right)^\intercal \\
& \btheta^{(k+1)}  = \btheta^{(k)} -\eta \left[ \bsg^{(k)}(\bsf^{(k)} - \bsr )\right]\\
\end{aligned}
\]
Inspired by Lemma B.2 in \cite{zhou2020neural} , we define the auxiliary sequence following :
\[
\wbtheta^{(0)} = \btheta^{(0)}, \ \ \wbtheta^{(k+1)}   = \wbtheta^{(k)} - \eta\left[ \bsg^{(0)} \left( [\bsg^{(0)}]^\intercal (\wbtheta^{(k)}  - \wbtheta^{(0)}) - \bsr \right)  +  m\lambda (\wbtheta^{(k)} - \wbtheta^{(0)} )  \right] 
\]
\end{definition}












































\begin{lemma}\label{lemma:subg}
In a round $t$, at $k$-th iteration of gradient descent, with probability at least
$1 - O(pL) e^{-\Omega(m)}$, we have
\[
\begin{aligned}
(1) \|\bsg^{(0)}\|_F & \leq \sqrt{t(L+1)} \sqrt{p}(C_1\mu\sqrt{q})^L/m \\
(2) \|\bsg^{(k)} - \bsg^{(0)}\|_F & \leq \sqrt{tq(L+1})  \Psi_{L, (k')}  ( (C_1\mu)^L + 2) \\
(2)  \|\mathbf{f}^{k} - {\bsg^{(0)}}^\intercal ( \btheta^{(k)} - \btheta^{(0)} )\|_2 &\leq \sqrt{t} \left( \Psi_{L, (k')} (C_2  + 1)  +  (C_1\mu)^L C_2 + \sqrt{q} w((L-1)  (C_1\mu)^L  + 1)  \right) /\sqrt{m}.
\end{aligned}
\]
\end{lemma}













\begin{lemma} \label{lemma:2thetab}
In a round $t$, at $k$-th iteration of gradient descent, with probability at least
$1 - O(pL) e^{-\Omega(m)}$, we have
\[
\begin{aligned}
& (1) \| \wbtheta^{(k)} - \btheta^{(0)} - \btheta_0'/\sqrt{m} \|_2  \leq \sqrt{\frac{t}{m \lambda}}  \\
 (2)  \| \widehat{\btheta}_{t} - \widehat{\btheta}_0 \|_F &  \leq   \frac{t(L+1) }{m}  \left( 2\sqrt{p}(C_1\mu\sqrt{q})^L/m +   \sqrt{q} \Psi_{L, (k')}  ( (C_1\mu)^L + 2) \right)    \sqrt{q}\Psi_{L, (k')}  ( (C_1\mu)^L + 2)    .
\end{aligned}
\]
\end{lemma}




\noindent \textbf{Proof of Lemma 6.2}
\[
\begin{aligned}
&\| \wbtheta^{(k+1)} - \btheta^{(k+1)} \|_2  \\
= & \|  \wbtheta^{(k)} - \btheta^{(k)}  - \eta\left[ \bsg^{(0)} \left( [\bsg^{(0)}]^\intercal (\wbtheta^{(k)}   - \btheta^{(k)} +  \btheta^{(k)} - \wbtheta^{(0)}) - \bsr \right)  +  m\lambda (\wbtheta^{(k)} - \btheta^{(k)} +  \btheta^{(k)} - \wbtheta^{(0)} ) \right]   \\
& +  \eta \left[ \bsg^{(k)}(\bsf^{(k)} - \bsr )\right]    \|  \\
=&  \| (1-\eta m\lambda) (\btheta^{(k)} -  \wbtheta^{(k)}) 
+ \eta (\bsg^{(k)} - \bsg^{(0)})(\bsf^{k} -\bsr) - \eta \bsg^{(0)} \left( \bsf^{(k)} 
-  [\bsg^{0}]^{\intercal} (\btheta^{(k)} - \btheta^{(0)}) \right) \\
& - \eta \bsg^{(0)}{\bsg^{(0)}}^\intercal  (\btheta^{(k)} -  \wbtheta^{(k)})    - \eta m\lambda   (\btheta^{(k)} - \btheta^{(0)})  \|_2 \\
\leq &  \eta \| (\bsg^{(k)} - \bsg^{(0)})(\bsf^{(k)} -\bsr)   \|_2
+ \eta \| \bsg^{(0)} \|_2\|\bsf^{(k)} -  [\bsg^{0}]^{\intercal} (\btheta^{(k)} - \btheta^{(0)})   \|_2  \\
&+ \eta \lambda \| \btheta^{(k)} - \btheta^{(0)}\|_2 + \left\| \mathbf{I} - \eta(m\lambda \mathbf{I} +  \bsg^{(0)}{\bsg^{(0)}}^\intercal )   \right\|_2 \| \btheta^{(k)} - \wbtheta^{(k)}\|_2 \\
=& A_1 + A_2 + A_3 + A_4
\end{aligned}
\] 
For $A_1$, by Lemma \ref{lemma:subg}, we have 
\[
A_1 \leq \eta \|\bsg^{(k)} - \bsg^{(0)}\|_2 \| \bsf^{(k)} - \bsr\|_2 \leq \eta  \sqrt{tq(L+1})  \Psi_{L, (k')}  ( (C_1\mu)^L + 2)  \sqrt{2t}  = \eta \bar{A}_1
\]
For $A_2$, by Lemma \ref{lemma:subg}, we have
\[
A_2 \leq \eta   t \sqrt{(L+1)} \sqrt{p}(C_1\mu\sqrt{q})^L \cdot \sqrt{t}  \left(  \Psi_{L, (k')} (C_2  + 1)  +  (C_1\mu)^L C_2 + \sqrt{q} w((L-1)  (C_1\mu)^L  + 1)  \right) m^{-3/2} = \eta \bar{A}_2.
\]
For $A_3$, by Lemma \ref{lemma:subg} and Lemma \ref{lemma:f-g0}, we have 
\[
A_3  \leq  (1 - \eta m \lambda) \| \btheta^{(k)} - \wbtheta^{(k)}\|_2   
\]
because $\mathbf{I} - \eta(m\lambda \mathbf{I} +  \bsg^{(0)}{\bsg^{(0)}}^\intercal ) \preceq \mathbf{I} -  \eta(m\lambda \mathbf{I} +  \left( \sqrt{t(L+1)} \sqrt{p}(C_1\mu\sqrt{q})^L/m \right)^2  \mathbf{I}) \preceq \mathbf{I}$ with the choice of $m$ and $\eta$.

For $A_3$, by Lemma \ref{lemma:wbound}, we have
\[
\eta \lambda \| \btheta^{(k)} - \btheta^{(0)}\|_2 = \eta \lambda  \sqrt{\sum_{l=1}^{L+1} \|\bw^{l, (k)} - \bw^{l, (0)}\|_F^2} =  \eta \lambda \sqrt{L+1}w/ \sqrt{m} = \eta \bar{A}_3.
\]


Therefore, adding everything together, we have 
\[
\| \btheta^{(k+1)} - \wbtheta^{(k+1)}\|_2 \leq  (1 - \eta m \lambda) \| \btheta^{(k)} - \wbtheta^{(k)}\|_2  +  \eta \bar{A}_1 +  \eta  \bar{A}_2+ \eta \bar{A}_3.
\]
As $\|\btheta^{(0)} - \wbtheta^{(0)}\| = 0$, by induction, we have
\[
\| \btheta^{(k)} - \wbtheta^{(k)}\|_2 \leq \frac{  \eta \bar{A}_1 +  \eta \bar{A}_2+  \eta \bar{A}_3 }{ \eta m \lambda } \leq \frac{   \bar{A}_1 +  \bar{A}_2+ \bar{A}_3 }{ m \lambda }
\]
By Lemma \ref{lemma:2thetab}, we have
\[
\begin{aligned}
\| \btheta^{(k)} - \btheta^{(0)} -  \widehat{\btheta}_t /\sqrt{m}\|_2 = & \| \btheta^{(k)} - \wbtheta^{(k)} + \wbtheta^{(k)} - \btheta^{(0)} - \widehat{\btheta}_0/\sqrt{m} + \widehat{\btheta}_0/\sqrt{m} - \widehat{\btheta}_t /\sqrt{m}\|_2\\
\leq &   \| \btheta^{(k)} - \wbtheta^{(k)}     \|_2 +  \| \wbtheta^{(k)} - \btheta^{(0)} - \widehat{\btheta}_0/\sqrt{m}  \|_2 +  \| \widehat{\btheta}_t - \widehat{\btheta}_0\|_2 /\sqrt{m}\\
\leq & \frac{  \bar{A}_1 +  \bar{A}_2+ \bar{A}_3 }{  m \lambda  } + \sqrt{  \frac{t}{m\lambda} }
\\ 
& + \frac{t(L+1) }{m}  \left( 2\sqrt{p}(C_1\mu\sqrt{q})^L/m +   \sqrt{q} \Psi_{L, (k')}  ( (C_1\mu)^L + 2) \right)    \sqrt{q}\Psi_{L, (k')}  ( (C_1\mu)^L + 2)    . 
\end{aligned}
\]

The proof is completed.
\qed
























